The Minimal Genus of Homology Classes in a Finite 2-Complex

We study surface representatives of homology classes of finite complexes which minimize certain complexity measures, including its genus and Euler characteristic. Our main result is that up to surgery at nullhomotopic curves minimizers are homotopic to cellwise coverings to the 2-skeleton. From this we conclude that the minimizing problem is in general algorithmically undecidable, but can be solved for 2-dimensional CAT(-1)-complexes.

==> Corollary/CellwiseCovering.Proof.tex <==
\begin{proof}[Proof of Corollary~\ref{crl:CellwiseCovering}]
  For every $\left(\Surface,\ContinuousMap\right)$ there exists a
  $\left(\Surface',\ContinuousMap'\right)$ such that
  $
    \left(\Surface',\ContinuousMap'\right)
    \CompressionSmallerEqual
    \left(\Surface,\ContinuousMap\right)
  $
  and $\ContinuousMap'$ admits no squeezes.
  By Theorem~\ref{thm:NormalForm}, this implies that $\ContinuousMap'$
  is homotopic to a cellwise covering without folds.
\end{proof}


==> Corollary/CellwiseCovering.tex <==
\begin{corollary}[Representing minimizers by cellwise coverings]%
\label{crl:CellwiseCovering}
  Given a generalized $2$-complex $X$ and a second homology class
  $
    \HomologyClass
    \in
    \HomologyOfSpaceObject{\TopologicalSpace}{2}
  $,
  then for every
  $
    \left(
      \Surface
      ,
      \ContinuousMap
    \right)
  $
  representing $\HomologyClass$ there exists a new representative
  $
    \left(
      \Surface',\ContinuousMap'
    \right)
  $ such that
  $
    \left(
      \Surface',\ContinuousMap'
    \right)
    \CompressionSmallerEqual
    \left(
      \Surface,\ContinuousMap
    \right)
  $
  and $\ContinuousMap'$ is a cellwise covering without folds.
\end{corollary}


==> Makefile <==
figuresInput=$(wildcard Figures/*.svg)
figuresOutput=$(figuresInput:.svg=.pdf_tex)
texSources=$(wildcard *.tex */*.tex)

all: pdf

%.pdf_tex: %.svg
	inkscape -z -D --file=$< --export-pdf=$(<:.svg=.pdf) --export-latex && \
	sed -i 's@{\([^{.]*.pdf\)}@{Figures/\1}@' $@

pdf: top.pdf

view: pdf
	evince top.pdf

top.pdf: $(figuresOutput) $(texSources)
	pdflatex top.tex
	bibtex top.aux
	pdflatex top.tex
	pdflatex top.tex

spellcheck: $(texSources)
	for file in $^; do aspell --lang=en_US --home-dir=. -t check $$file; done

clean:
	rm -rf top.aux top.log top.out top.blg top.bbl top.pdf Figures/*.pdf Figures/*.pdf_tex

style: $(texSources)
	for file in $^; do sed -i -e's@\s*$$@@' $$file; done

.PHONY: clean style spellcheck

